CATER: Intellectual Property Protection on Text Generation APIs via Conditional Watermarks

Previous works have validated that text generation APIs can be stolen through imitation attacks, causing IP violations. In order to protect the IP of text generation APIs, a recent work has introduced a watermarking algorithm and utilized the null-hypothesis test as a post-hoc ownership verification on the imitation models. However, we find that it is possible to detect those watermarks via sufficient statistics of the frequencies of candidate watermarking words. To address this drawback, in this paper, we propose a novel Conditional wATERmarking framework (CATER) for protecting the IP of text generation APIs. An optimization method is proposed to decide the watermarking rules that can minimize the distortion of overall word distributions while maximizing the change of conditional word selections. Theoretically, we prove that it is infeasible for even the savviest attacker (they know how CATER works) to reveal the used watermarks from a large pool of potential word pairs based on statistical inspection. Empirically, we observe that high-order conditions lead to an exponential growth of suspicious (unused) watermarks, making our crafted watermarks more stealthy. In addition, \cater can effectively identify the IP infringement under architectural mismatch and cross-domain imitation attacks, with negligible impairments on the generation quality of victim APIs. We envision our work as a milestone for stealthily protecting the IP of text generation APIs.

==> tab-data.tex <==
\begin{table}[h]
    \centering
     \caption{Statistics of datasets used in our experiments.}% on WMT14, IWSLT 2014 and OPUS (Law)
    \begin{tabular}{llll}
    \toprule
          & Train & Dev & Test\\
          \midrule
    WMT14 & 4.5M & 3K & 3003 \\
    CNN/DM & 287K & 13K  &  11K\\
    \bottomrule
    \end{tabular}
    %\vspace{-2mm}
    \label{tab:data}
    % \vspace{-4.0mm}
\end{table}
